Non normal logics: semantic analysis and proof theory

We introduce proper display calculi for basic monotonic modal logic,the conditional logic CK and a number of their axiomatic extensions. These calculi are sound, complete, conservative and enjoy cut elimination and subformula property. Our proposal applies the multi-type methodology in the design of display calculi, starting from a semantic analysis based on the translation from monotonic modal logic to normal bi-modal logic.

==> Properties.tex <==
\section{Properties}

Completeness of MML and its axiomatic extensions.

\begin{itemize}
\item[M] $\abla (A \wedge B) \rightarrow \abla A \wedge \abla B \quad \rightsquigarrow \quad \xdianu \dboxni (A \wedge B) \rightarrow \xdianu \dboxni A \wedge \xdianu \dboxni B$

\begin{center}
{\fns
\AX$A \fCenter A$
\UI$A \XAND B \fCenter A$
\UI$\dboxni (A \XAND B) \fCenter \DBOXNI A$
\UI$\dboxni (A \XAND B) \fCenter \dboxni A$
\UI$\XDIANU \dboxni (A \XAND B) \fCenter \xdianu \dboxni A$
\UI$\xdianu \dboxni (A \XAND B) \fCenter \xdianu \dboxni A$
%
\AX$B \fCenter B$
\UI$A \XAND B \fCenter B$
\UI$\dboxni (A \XAND B) \fCenter \DBOXNI B$
\UI$\dboxni (A \XAND B) \fCenter \dboxni B$
\UI$\XDIANU \dboxni (A \XAND B) \fCenter \xdianu \dboxni B$
\UI$\xdianu \dboxni (A \XAND B) \fCenter \xdianu \dboxni B$
%
\BI$\xdianu \dboxni (A \XAND B) \XAND \xdianu \dboxni (A \XAND B) \fCenter \xdianu \dboxni A \xand \xdianu \dboxni B$
\LL{\scs $C$}
\UI$\xdianu \dboxni (A \XAND B) \fCenter \xdianu \dboxni A \xand \xdianu \dboxni B$
\DP
}
\end{center}

\item[C] $\abla A \wedge \abla B \to \abla (A \wedge B) \quad \rightsquigarrow \quad \xdianu \dboxni A \wedge \xdianu \dboxni B \to \xdianu \dboxni (A \wedge B)$

\marginnote{Is $\XAND\XDIAIN$ sound??? ...we do not need it to derive axiom C: see the derivation on the right.}
\begin{center}
{\fns
\begin{tabular}{cc}
\AX$A \fCenter A$
\UI$\dboxni A \fCenter \DBOXNI A$
\UI$\XDIAIN \dboxni A \fCenter A$
%
\AX$B \fCenter B$
\UI$\dboxni B \fCenter \DBOXNI B$
\UI$\XDIAIN \dboxni B \fCenter B$
%
\BI$\XDIAIN \dboxni A \XAND \XDIAIN \dboxni B \fCenter A \XAND B$
\UI$\XDIAIN \dboxni A \XAND \XDIAIN \dboxni B \fCenter A \xand B$
\LL{\scs $\XAND\XDIAIN$}
\UI$\XDIAIN (\dboxni A \DAND \dboxni B) \fCenter A \xand B$
\UI$\dboxni A \DAND \dboxni B \fCenter \DBOXNI (A \xand B)$
\UI$\dboxni A \DAND \dboxni B \fCenter \dboxni (A \xand B)$
\UI$\XDIANU (\dboxni A \DAND \dboxni B) \fCenter \xdianu \dboxni (A \xand B)$
\LL{\scs $\XDIANU\XAND$}
\UI$\XDIANU \dboxni A \XAND \XDIANU \dboxni B \fCenter \xdianu \dboxni (A \xand B)$
\dashedLine
\UI$\xdianu \dboxni A \xand \xdianu \dboxni B \fCenter \xdianu \dboxni (A \xand B)$
\DP
 & 
\AX$A \fCenter A$
\UI$\dboxni A \fCenter \DBOXNI A$
\LL{\scs $W$}
\UI$\dboxni A \DAND \dboxni B \fCenter \DBOXNI A$
\UI$\XDIAIN (\dboxni A \DAND \dboxni B )\fCenter A$
%
\AX$B \fCenter B$
\UI$\dboxni B \fCenter \DBOXNI B$
\LL{\scs $W$}
\UI$\dboxni A \DAND \dboxni B \fCenter \DBOXNI B$
\UI$\XDIAIN (\dboxni A \DAND \dboxni B)\fCenter B$

%
\BI$\XDIAIN (\dboxni A \DAND \dboxni B) \XAND \XDIAIN (\dboxni A \DAND \dboxni B) \fCenter A \XAND B$
\LL{\scs $C$}
\UI$\XDIAIN (\dboxni A \DAND \dboxni B) \fCenter A \XAND B$
\UI$\dboxni A \DAND \dboxni B \fCenter \DBOXNI (A \xand B)$
\UI$\dboxni A \DAND \dboxni B \fCenter \dboxni (A \xand B)$
\UI$\XDIANU (\dboxni A \DAND \dboxni B) \fCenter \xdianu \dboxni (A \xand B)$
\LL{\scs $\XDIANU\XAND$}
\UI$\XDIANU \dboxni A \XAND \XDIANU \dboxni B \fCenter \xdianu \dboxni (A \xand B)$
\dashedLine
\UI$\xdianu \dboxni A \xand \xdianu \dboxni B \fCenter \xdianu \dboxni (A \xand B)$
\DP
 \\
\end{tabular}
}
\end{center}


\item[N] $\abla \top \quad \rightsquigarrow \quad \xdianu \dboxni \top$

\begin{center}
{\fns
\AX$\XTOP \fCenter \xtop$
\LL{\scs $\XTOP\XDIAIN$}
\UI$\XDIAIN \DTOP \fCenter \xtop$
\UI$\DTOP \fCenter \DBOXNI \xtop$
\UI$\DTOP \fCenter \dboxni \xtop$
\UI$\XDIANU \DTOP \fCenter \xdianu \dboxni \xtop$
\LL{\scs $\XDIANU\XTOP$}
\UI$\XTOP \fCenter \xdianu \dboxni \xtop$
\DP
}
\end{center}

\item[4] $\abla \abla A \xrarr \abla A \quad \rightsquigarrow \quad \xdianu \dboxni \xdianu \dboxni A \xrarr \xdianu \dboxni A$

\begin{center}
{\fns
\AX$A \fCenter A$
\UI$\dboxni A \fCenter \DBOXNI A$
\UI$\dboxni A \fCenter \dboxni A$
\LL{\scs ??? not sound $\XDIANU-\XBOXIN$}
\UI$\XDIANU \dboxni A \fCenter \XBOXIN \dboxni A$
\UI$\xdianu \dboxni A \fCenter \XBOXIN \dboxni A$
\UI$\dboxni \xdianu \dboxni A \fCenter \DBOXNI \XBOXIN \dboxni A$
\UI$\XDIAIN \dboxni \xdianu \dboxni A \fCenter \XBOXIN \dboxni A$
\UI$\DDIANI \XDIAIN \dboxni \xdianu \dboxni A \fCenter \dboxni A$
\UI$\XDIANU \DDIANI \XDIAIN \dboxni \xdianu \dboxni A \fCenter \xdianu \dboxni A$
\LL{\scs ??? $(\XDIANU\DDIANI\XDIAIN)\XDIANU$}
\UI$\XDIANU \dboxni \xdianu \dboxni A \fCenter \xdianu \dboxni A$
\UI$\xdianu \dboxni \xdianu \dboxni A \fCenter \xdianu \dboxni A$
\DP
}
\end{center}

In the following derivation we expand the language with $\dboxni_1$, $\DBOXNI_1$ and its adjoint $\XDIAIN_1$. Moreover we have an additional neighbourhood type $N_1$. This machinery could help to ``count'' the nesting of operators modulo a change of types (see 1-step algebras of Ghilardi et al.).

\begin{center}
{\fns
\AX$A \fCenter_{\!\!S\ } A$
\UI$\dboxni A \fCenter_{\!\!N\ } \DBOXNI A$
\UI$\dboxni A \fCenter_{\!\!N\ } \dboxni A$
\UI$\XDIANU \dboxni A \fCenter_{\!\!S\ } \xdianu \dboxni A$
\UI$\xdianu \dboxni A \fCenter_{\!\!S\ } \xdianu \dboxni A$
\UI$\dboxni_1 \xdianu \dboxni A \fCenter_{\!\!N1\ } \DBOXNI_1 \xdianu \dboxni A$
\UI$\XDIAIN_1 \dboxni_1 \xdianu \dboxni A \fCenter_{\!\!S\ } \xdianu \dboxni A$
\LL{\scs $\XDIAIN_1\XDIANU$}
\UI$\XDIANU \dboxni_1 \xdianu \dboxni A \fCenter_{\!\!S\ } \xdianu \dboxni A$
\UI$\xdianu \dboxni_1 \xdianu \dboxni A \fCenter_{\!\!S\ } \xdianu \dboxni A$
\DP
}
\end{center}

Monotone case
\item[R] $\abla A \xrarr A\quad \rightsquigarrow \quad \xdianu \dboxni A \xrarr A$

{\fns
\begin{center}
\begin{tabular}{c}
\AX$A \fCenter A$
\UI$\dboxni A \fCenter \DBOXNI A$
\UI$\XDIAIN \dboxni A \fCenter A$
\LL{\scs $\XDIAIN\XDIANU$}
\UI$\XDIANU \dboxni A \fCenter A$
\UI$\xdianu \dboxni A \fCenter A$
\DP
 \\
\end{tabular}
\end{center}
}


Non-monotone case 

\item[R] $\abla A \xrarr A\quad \rightsquigarrow \quad \xdianu (\dboxni A \dand \drhdnni A) \xrarr A$

{\fns
\begin{center}
\begin{tabular}{c}
\AX$A \fCenter A$
\UI$\dboxni A \fCenter \DBOXNI A$
\LL{\scs $W$}
\UI$\dboxni A \DAND \drhdnni A \fCenter \DBOXNI A$
\UI$\dboxni A \dand \drhdnni A \fCenter \DBOXNI A$
\UI$\XDIAIN (\dboxni A \dand \drhdnni A) \fCenter A$
\LL{\scs $\XDIAIN\XDIANU$}
\UI$\XDIANU (\dboxni A \dand \drhdnni A) \fCenter A$
\UI$\xdianu (\dboxni A \dand \drhdnni A) \fCenter A$
\DP
 \\
\end{tabular}
\end{center}
}

\end{itemize}

Completeness of CL and its axiomatic extensions.

\begin{itemize}
\item MP $(A > B) \xrarr (A \xrarr B) \quad \rightsquigarrow \quad ((\dboxni A \dand \drhdnni A) \mtra B) \xrarr (A \xrarr B)$ 

{\fns
\begin{center}
\begin{tabular}{c}
\AX$A \fCenter A$
\dboxni 
\AX$B \fCenter B$
\BI$ \fCenter B $
\DP
 \\
\end{tabular}
\end{center}
}
In the following derivations the rule $\XDIAIN\XAND\MTAND$ is too strong. In the derivation of CS, we should take into account that three occurrences of $A$ have to be the same and the two occurrences of $B$ have to be same. In the derivation of ID, we should take into account that the three occurrences of A have to be the same. If in the translation we could make use of $\ddiani, \dlhdnni$ instead of $\dboxni, \drhdnni$, we would be in a slightly better position. The problem is that we cannot access what is under the scope of a g-operator in precedent position via structural rule. 

\item CS $(A \xand B) \xrarr (A > B) \quad \rightsquigarrow \quad (A \xand B) \xrarr ((\dboxni A \dand \drhdnni A) \mtra B)$ 

{\fns
\begin{center}
\begin{tabular}{c}
\AX$B \fCenter B$
\LL{\scs $W$}
\UI$A \XAND B\fCenter B$
\UI$A \xand B\fCenter B$
\UI$A \xand B \XAND A\fCenter B$
\UI$A\fCenter (\XNEG A \xand B) \XOR B$
\UI$\dboxni A \fCenter \DBOXNI ((\XNEG A \xand B) \XOR B)$
\LL{\scs $W$}
\UI$\dboxni A \DAND \drhdnni A \fCenter \DBOXNI ((\XNEG A \xand B) \XOR B)$
\UI$\XDIAIN (\dboxni A \dand \drhdnni A) \fCenter (\XNEG A \xand B) \XOR B$
\UI$(A \xand B) \XAND \XDIAIN (\dboxni A \dand \drhdnni A) \fCenter B$
\UI$\XDIAIN (\dboxni A \dand \drhdnni A) \XAND (A \xand B) \fCenter B$
\LL{\scs $\XDIAIN\XAND\MTAND$}
\UI$(\dboxni A \dand \drhdnni A) \MTAND (A \xand B) \fCenter B$
\UI$A \xand B \fCenter (\dboxni A \dand \drhdnni A) \MTRA B$
\UI$A \xand B \fCenter (\dboxni A \dand \drhdnni A) \mtra B$
\DP
\end{tabular}
\end{center}
}

\item ID $A > A \quad \rightsquigarrow \quad (\dboxni A \dand \drhdnni A) \mtra A$

{\fns
\begin{center}
\begin{tabular}{c}
\AX$A \fCenter A$
\UI$\dboxni A \fCenter \DBOXNI A$
\LL{\scs $W$}
\UI$\dboxni A \DAND \drhdnni A \fCenter \DBOXNI A$
\UI$\dboxni A \dand \drhdnni A \fCenter \DBOXNI A$
\UI$\XDIAIN (\dboxni A \dand \drhdnni A) \fCenter A$
\LL{\scs $\XTOP$}
\UI$\XDIAIN (\dboxni A \dand \drhdnni A) \XAND \XTOP \fCenter A$
\LL{\scs $\XDIAIN\XAND\MTAND$}
\UI$(\dboxni A \dand \drhdnni A) \MTAND \XTOP \fCenter A$
\UI$\XTOP \fCenter (\dboxni A \dand \drhdnni A) \MTRA A$
\UI$\XTOP \fCenter (\dboxni A \dand \drhdnni A) \mtra A$
\DP
\end{tabular}
\end{center}
}

\item CEM $(A > B) \xor (A > \xneg B) \quad \rightsquigarrow \quad ((\dboxni A \dand \drhdnni A) \mtra B) \xor ((\dboxni A \dand \drhdnni A) \mtra \xneg B)$


\end{itemize}




==> macros.tex <==
%%%theorem styles

%%%theorem styles

\newtheorem{theorem}{Theorem}[section]
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{note}[theorem]{Note}
\newtheorem{counterexample}[theorem]{Counterexample}
\newtheorem{conjecture}[theorem]{Conjecture}
\newtheorem{notation}[theorem]{Notation}
\newtheorem{fact}[theorem]{Fact}
\newtheorem{example}[theorem]{Example}

\newtheorem{definition}[theorem]{Definition}

\newtheorem{remark}[theorem]{Remark}

\def\fCenter{{\mbox{$\ \vdash\ $}}}

%%%Editing helps

%\newcommand{\comment}[1]{}

\newcommand{\fns}{\footnotesize}

\newcommand{\marginnote}[1]{\marginpar{\raggedright\tiny{#1}}}

\newcommand{\marginredbf}[1]{\marginnote{\redbf{#1}}}

\def\mc{\multicolumn}

\newcommand{\todoA}[1]{\textnormal{\color{red}\scriptsize+++A: #1+++}}
\newcommand{\todoB}[1]{\textnormal{\color{blue}\scriptsize +++B: #1+++}}
\newcommand{\todoC}[1]{\textnormal{\color{Green}\scriptsize +++C: #1+++}} 

%Distributive Lattice
%Operational Connectives
\newcommand{\xtop}{\ensuremath{\top}\xspace}
\newcommand{\xbot}{\ensuremath{\bot}\xspace}
\newcommand{\xand}{\ensuremath{\wedge}\xspace}
\newcommand{\xor}{\ensuremath{\vee}\xspace}
\newcommand{\xrarr}{\ensuremath{\rightarrow}\xspace}
\newcommand{\xcrarr}{\ensuremath{\,{>\mkern-7mu\raisebox{-0.065ex}{\rule[0.5865ex]{1.38ex}{0.1ex}}}\,}\xspace}
%Structural Connectives
\newcommand{\XTOP}{\ensuremath{\hat{\top}}\xspace}
\newcommand{\XBOT}{\ensuremath{\check{\bot}}\xspace}
\newcommand{\XAND}{\ensuremath{\:\hat{\wedge}\:}\xspace}
\newcommand{\XOR}{\ensuremath{\:\check{\vee}\:}\xspace}
\newcommand{\XRARR}{\ensuremath{\:\check{\rightarrow}\:}\xspace}
\newcommand{\XCRARR}{\ensuremath{\hat{{\:{>\mkern-7mu\raisebox{-0.065ex}{\rule[0.5865ex]{1.38ex}{0.1ex}}}\:}}}\xspace}



\newcommand{\topic}{\ensuremath{\mathrm{t}}\xspace}
\newcommand{\botic}{\ensuremath{\mathrm{f}}\xspace}

%Neighobourood
%Operational Connectives
\newcommand{\nneg}{\ensuremath{{\sim}}\xspace}
\newcommand{\nrneg}{\ensuremath{\neg}\xspace}
\newcommand{\ntop}{\ensuremath{1}\xspace}
\newcommand{\nbot}{\ensuremath{0}\xspace}
\newcommand{\nand}{\ensuremath{\cap}\xspace}
\newcommand{\nor}{\ensuremath{\cup}\xspace}
\newcommand{\nrarr}{\ensuremath{>}\xspace}
\newcommand{\ncrarr}{\ensuremath{\,{>\mkern-7mu\raisebox{-0.065ex}{\rule[0.5865ex]{1.38ex}{0.1ex}}}\,}\xspace}
%Structural Connectives
%\newcommand{\NNEG}{\ensuremath{*}\xspace}
\newcommand{\NNEG}{\ensuremath{\circledast}\xspace}
\newcommand{\NTOP}{\ensuremath{\hat{1}}\xspace}
\newcommand{\NBOT}{\ensuremath{\check{0}}\xspace}
\newcommand{\NAND}{\ensuremath{\:\hat{\cap}\:}\xspace}
\newcommand{\NOR}{\ensuremath{\:\check{\cup}\:}\xspace}
\newcommand{\NRARR}{\ensuremath{\:\check{>}\:}\xspace}
\newcommand{\NCRARR}{\ensuremath{\hat{{\:{>\mkern-7mu\raisebox{-0.065ex}{\rule[0.5865ex]{1.38ex}{0.1ex}}}\:}}}\xspace}

%OLD Heterogeneous connectives
%OLD Operational connectives
\newcommand{\wbox}{\ensuremath{\Box}\xspace}
\newcommand{\wdia}{\ensuremath{\Diamonddot}\xspace}
\newcommand{\bcirc}{\ensuremath{{\bullet}}\xspace}
\newcommand{\bbox}{\ensuremath{\boxdot}\xspace}
\newcommand{\bdia}{\ensuremath{\Diamondblack}\xspace}
%OLD Structural connectives
\newcommand{\WBOX}{\ensuremath{\:\check{\Box}\:}\xspace}
\newcommand{\WDIA}{\ensuremath{\:\hat{\Diamond}}\xspace}
\newcommand{\BBOX}{\ensuremath{\:\check{\blacksquare}}\xspace}
\newcommand{\BDIA}{\ensuremath{\:\hat{\Diamondblack}}\xspace}
\newcommand{\WCIR}{\ensuremath{\:\tilde{{\circ}}}\xspace}
\newcommand{\BCIR}{\ensuremath{\:\tilde{{\bullet}}}\xspace}

%Heterogeneous connectives
%Operational connectives
\newcommand{\XDIANU}{\ensuremath{\langle\hat{\nu}\rangle}\xspace}
\newcommand{\xdianu}{\ensuremath{\langle\nu\rangle}\xspace}
\newcommand{\DBOXUN}{\ensuremath{[\check{\rotatebox[origin=c]{180}{$\nu$}}]}\xspace}
\newcommand{\dboxun}{\ensuremath{[\rotatebox[origin=c]{180}{$\nu$}]}\xspace}

\newcommand{\DDIANI}{\ensuremath{\langle\hat{\ni}\rangle}\xspace}
\newcommand{\ddiani}{\ensuremath{\langle\ni\rangle}\xspace}
\newcommand{\XBOXIN}{\ensuremath{[\check\in]}\xspace}
\newcommand{\xboxin}{\ensuremath{[\in]}\xspace}

\newcommand{\XDIAUN}{\ensuremath{\langle\hat{\rotatebox[origin=c]{180}{$\nu$}}\rangle}\xspace}
\newcommand{\xdiaun}{\ensuremath{\langle\rotatebox[origin=c]{180}{$\nu$}\rangle}\xspace}
\newcommand{\DBOXNU}{\ensuremath{[\check{\nu}]}\xspace}
\newcommand{\dboxnu}{\ensuremath{[\nu]}\xspace}

\newcommand{\DDIAIN}{\ensuremath{\langle\hat{\in}\rangle}\xspace}
\newcommand{\ddiain}{\ensuremath{\langle\in\rangle}\xspace}
\newcommand{\XBOXNI}{\ensuremath{[\check\ni]}\xspace}
\newcommand{\xboxni}{\ensuremath{[\ni]}\xspace}






==> macros_RA_.tex <==
%KI
%Operational Connectives
\newcommand{\Ineg}{\ensuremath{{\sim}}\,}
%\newcommand{\rdneg}{\ensuremath{\neg}\xspace}
%\newcommand{\Itop}{\ensuremath{1_\mathrm{I}}\xspace}
%\newcommand{\Ibot}{\ensuremath{0_\mathrm{I}}\xspace}
\newcommand{\Itop}{\ensuremath{1_I}\xspace}
\newcommand{\Ibot}{\ensuremath{0_I}\xspace}

\newcommand{\Iand}{\ensuremath{\cap}\xspace}
\newcommand{\Ior}{\ensuremath{\cup}\xspace}
\newcommand{\Irarr}{\ensuremath{\,{\raisebox{-0.065ex}{\rule[0.5865ex]{1.38ex}{0.1ex}}\mkern-5mu\supset}\,}\xspace}

\newcommand{\Icrarr}{\ensuremath{\,{\supset\mkern-5.5mu\raisebox{-0.065ex}{\rule[0.5865ex]{1.38ex}{0.1ex}}}\,}\xspace}
\newcommand{\Idrarr}{\ensuremath{\,{\supset\mkern-5.5mu\raisebox{-0.065ex}{\rule[0.5865ex]{1.38ex}{0.1ex}}}\,}\xspace}

%Structural Connectives
\newcommand{\INEG}{\,\ensuremath{\sim}\,\,}
\newcommand{\ADINEG}{\ensuremath{\circledast}\xspace}
%\newcommand{\ITOP}{\ensuremath{\hat{1}_\mathrm{I}}\xspace}
%\newcommand{\IBOT}{\ensuremath{\check{0}_\mathrm{I}}\xspace}
\newcommand{\ITOP}{\ensuremath{\hat{1}_I}\xspace}
\newcommand{\IBOT}{\ensuremath{\check{0}_I}\xspace}
\newcommand{\IAND}{\ensuremath{\:\hat{\cap}\:}\xspace}
\newcommand{\IOR}{\ensuremath{\:\check{\cup}\:}\xspace}
\newcommand{\IRARR}{\ensuremath{\check{\,{\raisebox{-0.065ex}{\rule[0.5865ex]{1.38ex}{0.1ex}}\mkern-5mu\supset}\,}}\xspace}
\newcommand{\ICRARR}{\ensuremath{\hat{\,{\supset\mkern-5.5mu\raisebox{-0.065ex}{\rule[0.5865ex]{1.38ex}{0.1ex}}}\,}}\xspace}
\newcommand{\IDRARR}{\ensuremath{\hat{\,{\supset\mkern-5.5mu\raisebox{-0.065ex}{\rule[0.5865ex]{1.38ex}{0.1ex}}}\,}}\xspace}

%KC
%Operational Connectives
\newcommand{\Cneg}{\,\ensuremath{-}\,\,}
\newcommand{\Ctop}{\ensuremath{1}_\mathrm{C}\,\xspace}
\newcommand{\Cbot}{\ensuremath{0}_\mathrm{C}\,\xspace}
\newcommand{\Cand}{\ensuremath{\sqcap}\xspace}
\newcommand{\Cor}{\ensuremath{\sqcup}\xspace}
\newcommand{\Crarr}{\ensuremath{\,{\raisebox{-0.065ex}{\rule[0.5865ex]{1.38ex}{0.1ex}}\mkern-5mu\sqsupset}\,}\xspace}
\newcommand{\Ccrarr}{\ensuremath{\,{\sqsupset\mkern-5.5mu\raisebox{-0.065ex}{\rule[0.5865ex]{1.38ex}{0.1ex}}}\,}\xspace}
\newcommand{\Cdrarr}{\ensuremath{\,{\sqsupset\mkern-5.5mu\raisebox{-0.065ex}{\rule[0.5865ex]{1.38ex}{0.1ex}}}\,}\xspace}

%Structural Connectives
\newcommand{\CNEG}{\,\ensuremath{\:\tilde{-}}\,\,}
\newcommand{\CADINEG}{\ensuremath{\circledast}\xspace}
%\newcommand{\CTOP}{\ensuremath{\hat{1}_\mathrm{C}}\xspace}
%\newcommand{\CBOT}{\ensuremath{\check{0}_\mathrm{C}}\xspace}
\newcommand{\CTOP}{\ensuremath{\hat{1}_C}\xspace}
\newcommand{\CBOT}{\ensuremath{\check{0}_C}\xspace}
\newcommand{\CAND}{\ensuremath{\:\hat{\sqcap}\:}\xspace}
\newcommand{\COR}{\ensuremath{\:\check{\sqcup}\:}\xspace}
\newcommand{\CRARR}{\ensuremath{\check{\,{\raisebox{-0.065ex}{\rule[0.5865ex]{1.38ex}{0.1ex}}\mkern-5mu\sqsupset}\,}}\xspace}
\newcommand{\CCRARR}{\ensuremath{\hat{\,{\sqsupset\mkern-5.5mu\raisebox{-0.065ex}{\rule[0.5865ex]{1.38ex}{0.1ex}}}\,}}\xspace}


%Heterogeneous connectives
%Operational connectives
\newcommand{\wbox}{\ensuremath{\circ}_C\xspace}
\newcommand{\wdia}{\ensuremath{\circ}_I\xspace}

\newcommand{\Cwcirc}{\ensuremath{\circ}_C\xspace}
\newcommand{\Iwcirc}{\ensuremath{\circ}_I\xspace}


\newcommand{\bcirc}{\ensuremath{{\bullet}}\xspace}
\newcommand{\adbboxl}{\ensuremath{\, \circ_l\,}\xspace}
\newcommand{\adbboxr}{\ensuremath{\: \circ_r\,}\xspace}

\newcommand{\bboxr}{\ensuremath{\blacksquare}_I\,\xspace}
\newcommand{\bboxl}{\ensuremath{\Diamondblack}_I\,\xspace}

\newcommand{\Ibbox}{\ensuremath{\blacksquare}_I\,\xspace}
\newcommand{\Ibdia}{\ensuremath{\Diamondblack}_I\,\xspace}

\newcommand{\bdiar}{\ensuremath{\blacksquare}_C\,\xspace}
\newcommand{\bdial}{\ensuremath{\Diamondblack}_C\,\xspace}

\newcommand{\Cbbox}{\ensuremath{\blacksquare}_C\,\xspace}
\newcommand{\Cbdia}{\ensuremath{\Diamondblack}_C\,\xspace}
%Structural connectives
\newcommand{\WBOX}{\ensuremath{\tilde{\circ}_C\,}\xspace}
\newcommand{\ADBBOXL}{\ensuremath{\:\hat{\circ}_l\,}\xspace}


\newcommand{\ADBBOXR}{\ensuremath{\:\check{\circ}_r\,}\xspace}
\newcommand{\WDIA}{\ensuremath{\:\tilde{\circ}_I\,}\xspace}

\newcommand{\BBOXR}{\ensuremath{\:\check{\blacksquare}_I\,}\xspace}
\newcommand{\BBOXL}{\ensuremath{\:\hat{\Diamondblack}_I\,}\xspace}
\newcommand{\BDIAL}{\ensuremath{\:\hat{\Diamondblack}_C\,}\xspace}
\newcommand{\BDIAR}{\ensuremath{\:\check{\blacksquare}_C\,}\xspace}

\newcommand{\WCIR}{\ensuremath{\:\tilde{{\circ}}}\xspace}
\newcommand{\BCIR}{\ensuremath{\:\tilde{{\bullet}}}\xspace}

